Learning to Represent Programs with Graphs

Learning tasks on source code (i.e., formal languages) have been considered recently, but most work has tried to transfer natural language methods and does not capitalize on the unique opportunities offered by code's known syntax. For example, long-range dependencies induced by using the same variable or function in distant locations are often not considered. We propose to use graphs to represent both the syntactic and semantic structure of code and use graph-based deep learning methods to learn to reason over program structures. In this work, we present how to construct graphs from source code and how to scale Gated Graph Neural Networks training to such large graphs. We evaluate our method on two tasks: VarNaming, in which a network attempts to predict the name of a variable given its usage, and VarMisuse, in which the network learns to reason about selecting the correct variable that should be used at a given program location. Our comparison to methods that use less structured program representations shows the advantages of modeling known structure, and suggests that our models learn to infer meaningful names and to solve the VarMisuse task in many cases. Additionally, our testing showed that VarMisuse identifies a number of bugs in mature open-source projects.

==> figures/computation.tex <==
\tikzset{computegraph/.style={
                    every node/.style={anchor=west, font=\tt,
                    text depth=0.5ex, text height=1.5ex, text centered, scale=.75,
                    inner sep=2pt},
                    knownplaceholder/.append style={rectangle, draw=red, color=black, minimum width=5ex},
                    placeholder/.append style={rectangle, draw=red,solid,line width=.5pt},
                    usagecx/.append style={rectangle, draw=blue, fill=blue!10, solid,line width=.5pt},
        }
}
\centering
\begin{subfigure}[b]{.45\textwidth}
\begin{minipage}{\textwidth}\centering
  \begin{tikzpicture}[computegraph]
    \node[knownplaceholder] (l0) at (0,0) {$\lambda_0$};
    \node[knownplaceholder] (l1) [right of=l0] {$\lambda_1$};
    \node[knownplaceholder] (l2) [right of=l1] {$\lambda_2$};
    \node[knownplaceholder] (l3) [right of=l2] {$\lambda_3$};
    
    \node[placeholder] (l4) [below of=l3] {$\lambda_4$};
    \node[placeholder] (l5) [below of=l1] {$\lambda_5$};

    \node[placeholder] (l7) [below of=l0] {$\lambda_7$};

    \node[usagecx] (beforearr) [below of=l7] {arr};
    
     \node[usagecx] (beforelim) [right of=beforearr] {lim};

     \node[usagecx] (beforesum) [right of=beforelim] {sum};    
    
    \node[usagecx] (beforei) [right of=beforesum] {i};    

    \node (beforetitle) [right of=beforei] {$\dataFlowIn{\lambda_8}{\var_i}$};
 
    % Unknown dataflow edges
     \draw[thick, blue, dotted]
      (l0.south) edge[->] (l7.north)
      (l7) edge[->] (beforearr)
      (l5) edge[->] (beforelim)
      (l4) edge[->] (beforei)
      (l2) edge[->] (beforesum)
      (l1.south) edge[->] (l5.north)  
      (l3.south) edge[->] (l4.north)
    ;

    \begin{scope}[on background layer]
      \draw[color=blue!30, dashed, rounded corners]
        ($(beforearr.north west) + (-0.13, 0.13)$)
        rectangle
        ($(beforetitle.south east) - (-0.13, 0.13)$);
    \end{scope}
  \end{tikzpicture}
\end{minipage}
\caption{$\dataFlowIn{\lambda_8}{\var_i}$ for in-scope variables at $\lambda_8$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[b]{.45\textwidth}
\begin{minipage}{\textwidth}\centering
  \begin{tikzpicture}[computegraph]
    \node[usagecx] (afterarr) at (0,0)  {arr};
    \node[usagecx] (afterlim) [right of=afterarr] {lim};    
    \node[usagecx] (aftersum) [right of=afterlim] {sum};
    \node[usagecx] (afteri) [right of=aftersum] {i};
    \node (aftertitle) [right of=afteri] {$\dataFlowOut{\lambda_8}{\var_i}$};

    \node[knownplaceholder, dashed] (empty) [below of=afterlim] {$\epsilon$};
    \node[placeholder] (l10) [left of=empty] {$\lambda_{10}$};
    \node[placeholder] (l9) [right of=empty] {$\lambda_{9}$}; 
    \node[knownplaceholder] (l12) [right of=l9] {$\lambda_{12}$};   
    \node[placeholder] (l11) [right of=l12] {$\lambda_{11}$};
    \node[placeholder] (l6) [right of=l11] {$\lambda_6$};


    % Unknown dataflow edges
     \draw[thick, blue, dotted] 
      (l12.south) edge[->, bend left=50] (l9.south)
      (l6.south) edge[->, bend left=50] (l11.south)
      (l10) edge[->] (afterarr)
      (l11) edge[->] (afteri)
      (l6) edge[->] (afteri)
      (l9) edge[->] (aftersum)
      (l12) edge[->] (aftersum)
     (empty) edge[->] (afterlim)
     (empty) edge[->] (afterarr) 
    ;

    \begin{scope}[on background layer]
      \draw[color=blue!30, dashed, rounded corners]
        ($(afterarr.north west) + (-0.13, 0.13)$)
        rectangle
        ($(aftertitle.south east) - (-0.13, 0.13)$);
    \end{scope}
  \end{tikzpicture}
\end{minipage}
\caption{$\dataFlowOut{\lambda_8}{\var_i}$ for in-scope variables at $\lambda_8$}
\end{subfigure}

==> figures/introfig.tex <==
\centering
\begin{subfigure}[b]{.54\textwidth}
\begin{minipage}{\textwidth}
\begin{lstlisting}[xleftmargin=0cm]
int SumPositive(int[] arr(*\hlref{0}*), int lim(*\hlref{1}*)) {
    int sum(*\hlref{2}*)=0;
   (*\hspace{-.8mm}\tikz[remember picture] \node [] (regStart) {};*)for(int i(*\hlref{3}*)=0; (*\hlplacehld{i}{4}*)<(*\hlplacehld{lim}{5}*); (*\hlplacehld{i}{6}*)++)
       if ((*\hlplacehld{arr}{7}*)[(*\hlplacehld{i}{8}*)]>0) (*\hlplacehld{sum}{9}*)+=(*\hlplacehld{arr}{10}*)[(*\hlplacehld{i}{11}*)];              (*\tikz[remember picture] \node [] (regEnd) {};*)
    return sum(*\hlref{12}*);
}
\end{lstlisting}
\begin{tikzpicture}[remember picture, overlay]
    \draw[draw=black, dashed, fill=green!40, rounded corners,fill opacity=.1] ($(regStart.north west) + (.1, .1)$) rectangle ($(regEnd.south) - (.1, .15)$);
\end{tikzpicture}
\end{minipage}
\caption{Example source code, with pasted snippet shaded in green.
  Tokens corresponding to variables marked by $\lambda_i$.
  The red boxes are the placeholders whose variable needs to be inferred 
  in the \varmisusetask{} task (ground truth variable
  name shown for convenience).}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[b]{.4\textwidth}
\begin{minipage}{\textwidth}
    \tikzset{placeholdergraph/.style={
                    every node/.style={anchor=west, font=\tt,
                    text depth=0.5ex, text height=1.5ex, text centered, scale=.75,
                    inner sep=2pt},
                    knownplaceholder/.append style={rectangle, draw=red, color=black},
                    placeholder/.append style={rectangle, fill=red!10,draw=red,solid,line width=.5pt},
            }
    }

  \begin{tikzpicture}[placeholdergraph, node distance=6pt and 5pt]
    \node[knownplaceholder] (l0) at (0,0) {$\lambda_0$:arr};
    \node[knownplaceholder] (l1) [right= of l0] {$\lambda_1$:lim};
    \node[knownplaceholder] (l3) [right= of l1] {$\lambda_3$:i};
    \node[knownplaceholder] (l2) [right= of l3] {$\lambda_2$:sum};
    
    \node[placeholder] (l4) [below=of l3] {$\lambda_4$:i};
    \node[placeholder] (l5) [below=of l1] {$\lambda_5$:lim};

    \node[placeholder] (l7) [below=of l0] {$\lambda_7$:arr};
    \node[placeholder] (l8) [below=of l5] {$\lambda_8$:i};

    \node[placeholder] (l11) [below=of l8] {$\lambda_{11}$:i};
    \node[placeholder] (l10) [left=of l11] {$\lambda_{10}$:arr};
    \node[placeholder] (l9) [right=of l11] {$\lambda_{9}$:sum};    
    \node[placeholder] (l6) [right=of l9] {$\lambda_6$:i};

    \node[knownplaceholder] (l12) [right=of l6] {$\lambda_{12}$:sum};

    % Known dataflow edges
    \draw[thick, dashed, blue]
      (l2.south east) edge[->, bend left=30] (l12.north)
    ;

    % Unknown dataflow edges
     \draw[thick, dotted, red]
      (l0.south) edge[->] (l7.north)
      (l1.south) edge[->] (l5.north)
      (l2.south) edge[->, bend right=5] (l9.north)   
      (l7.south) edge[->, bend right=5] (l10.north)  
      (l9.south) edge[->, bend right=40] (l12.south)
      (l3.south) edge[->] (l4.north)
      (l4.south) edge[->, bend left=13] (l8.east)
      (l8.south) edge[->] (l11.north)
      (l11.south) edge[->, bend right=40] (l6.south)
      (l8.east) edge[->, bend left=10] (l6.north)
    ;

    % The path edges
    % \draw
    %   (l0) edge[->] (l1)
    %   (l1) edge[->] (l2)
    %   (l2) edge[->] (l3)
    %   (l3) edge[->] (l4)
    %   (l4) edge[->] (l5)
    %   (l5) edge[->] (l7)
    %   (l5) edge[->] (l12)
    %   (l7) edge[->] (l8)      
    %   (l8) edge[->] (l10)
    %   (l8) edge[->, bend right=4] (l6)   
    %   (l10) edge[->] (l11)   
    %   (l11) edge[->] (l9)   
    %   (l9) edge[->] (l6)   
    %   (l6) edge[->] (l12)
    % ;
  \end{tikzpicture}
\end{minipage}
\caption{Dataflow diagram for variables in example, using ground truth
  placeholder choices.
  Dotted red edges show dataflow that depends on placeholder allocations.
  Dashed blue edge is dataflow independent of choices.\label{fig:smartpastegraph}}
\end{subfigure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> figures/nearestneighbors.tex <==
\begin{minipage}{\textwidth}
\begin{lstlisting}[frame=tlbr]

\end{lstlisting}
\end{minipage}\vspace{-1em}
\begin{minipage}{\textwidth}
\begin{lstlisting}[frame=tlbr]

\end{lstlisting}
\end{minipage}\vspace{-1em}
